BLEWhisperer: Exploiting BLE Advertisements for Data Exfiltration

Bluetooth technology has enabled short-range wireless communication for billions of devices. Bluetooth Low-Energy (BLE) variant aims at improving power consumption on battery-constrained devices. BLE-enabled devices broadcast information (e.g., as beacons) to nearby devices via advertisements. Unfortunately, such functionality can become a double-edged sword at the hands of attackers. In this paper, we primarily show how an attacker can exploit BLE advertisements to exfiltrate information from BLE-enable devices. In particular, our attack establishes a communication medium between two devices without requiring any prior authentication or pairing. We develop a proof-of-concept attack framework on the Android ecosystem and assess its performance via a thorough set of experiments. Our results indicate that such an exfiltration attack is indeed possible though with a limited data rate. Nevertheless, we also demonstrate potential use cases and enhancements to our attack that can further its severeness. Finally, we discuss possible countermeasures to prevent such an attack.

==> formats.tex <==
\IEEEPARstart{C}{ryptomining}, or simply mining, 
\par
\textit{Motivation:} A genuine ... 
\par
\ankit{Cybercriminals have made} ...
\par
To further aggravate the situation, ...
\par
\textit{Contribution:} In this paper, we focus on detecting covert cryptomining. The major contributions of this paper are as~follows:
\begin{enumerate}
	\item We propose a novel and efficient approach 
	
	\item We exhaustively assess the quality of our proposed approach with
	
	\item In the spirit of reproducible research, we make our collected datasets and the code publicly available\footnote{https://ciaoankit.github.io/abcd/}.
\end{enumerate}

\par
\textit{Organization:} The remainder of this paper is organized as follows. Section~\ref{section:related_work} presents a summary of the related works. We explain our system's architecture in Section~\ref{section:system_architecture} and discuss its evaluation in Section~\ref{section:evaluation}. Section~\ref{section:discussion} addresses the potential limitations of our proposed solution. Finally, Section~\ref{section:conclusion} concludes the paper.

\section{Related works}
\label{section:related_work}
HPC are .... generic malware~\cite{demme2013feasibility, yuan2011security, Wang:HPC}, kernel-level rootkits~\cite{wang2013numchecker}, side-channel attacks~\cite{chiappetta2016real}, unauthorized firmware modifications~\cite{wang2015confirm}\etc 
\par
\ankit{A general }
\par
\ankit{On another side, ... However, only a limited number of cryptocurrencies can be mined in the web-browsers. MineGuard~\cite{tahir2017mining} focuses on detecting cryptomining operations in the cloud~infrastructure.}
\par
\ankit{Our work is different from the state-of-the-art on the following dimensions: (1)~our proposed solution is a generic solution that is not tailored to a particular cryptocurrency or a specific form (e.g., browser-based) of cryptomining on computers; and (2)~we tested our solution against all the cryptocurrencies mined~by the top-10 mining pools, which collectively represent the largest portion of the cryptomining business.}

\section{System architecture}
\label{section:system_architecture}
We elucidate the key concept behind our approach in Section~\ref{section:core_concept}, our data collection phase in Section~\ref{section:data_collection}, selection of cryptocurrencies Section~\ref{section:cryptocurrencies_miners}, and our classifier's design in Section~\ref{section:classifier_design}.

\subsection{Fundamental intuition of our approach}
\label{section:core_concept}
The task of 

\subsection{Data collection}
\label{section:data_collection}	
To better explain our work, we first describe 

\subsection{Cryptocurrencies and miners}
\label{section:cryptocurrencies_miners}
The probability of solving the cryptographic
\subsection{Classifier design}
\label{section:classifier_design}
In this section, we elucidate the design of our classification methodology. Algorithm~\ref{algorithm:procedure} describes the pipeline of our~classifier. 

\begin{algorithm}[H]
	\caption{Pseudo code for our supervised classification.}
	\label{algorithm:procedure}
	%\hspace*{\algorithmicindent} \textbf{Input:} $S_{initial}$ 
	\begin{algorithmic}[1]
		%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
		%\renewcommand{\algorithmicensure}{\textbf{Output:}}
		%\REQUIRE \ankit{in}
		%\ENSURE  \ankit{out}
		
		\FOR{each run $i$ from 1 to 10}
		\STATE Create \textit{raw\_train\_set} and \textit{raw\_test\_set} by 90-10\% stratified partitioning.
		
		\STATE \textit{Data preprocessing}\\
		$\bullet$ Replace \textit{NaN} values from \textit{raw\_train\_set} and \textit{raw\_test\_set} with arithmetic mean of the considered event.
		
		\STATE \textit{Feature engineering}\\
		$\bullet$ \textit{train\_set} := Extract\_feature(\textit{raw\_train\_set})\\
		$\bullet$ \textit{test\_set} := Extract\_feature(\textit{raw\_test\_set})
		
		\STATE \textit{Feature scaling}\\
		%We chose StandardScaler as a scaler.
		$\bullet$ scaler := StandardScaler()\\
		$\bullet$ scaler.fit(\textit{train\_set}) \hfill $\rhd$\textit{Fit scaler on \textit{train\_set}}
		
		%\STATE \textit{Transform the \textit{train\_set} and \textit{test\_set} using \textit{scaler}}\\
		$\bullet$ scaler.transform(\textit{train\_set})\\
		$\bullet$ scaler.transform(\textit{test\_set})
		
		\STATE \textit{Feature selection}\\
		$\bullet$ Compute features' importance with \textit{forests of trees} on \textit{train\_set} and select the most relevant features. %with \textit{n\_estimators := 100} and \textit{max\_features := 50\%}
		
		\STATE \textit{Training}\\
		$\bullet$ Learn the model parameters for the given classifier (RF/SVM) on the training set using grid search with 5-fold stratified CV.
		%$\bullet$ Create and tune the model using grid search with 5-fold stratified CV.
		
		\STATE \textit{Predict/classify} the \textit{test\_set}.
		\ENDFOR			
	\end{algorithmic}
\end{algorithm}


\section{Evaluation}
\label{section:evaluation}
%	\section{Results}
%		\label{section:results}
We throughly evaluated our approach by performing an exhaustive set of experiments. 
\subsection{Binary classification}
\label{section:binary_classification}
Our main goal
\begin{table}[H]
	\centering
	\caption{Results for binary classification}
	\label{table:results_binary}
	\resizebox{.98\columnwidth}{!}
	{
		\begin{tabular}{|c|c|c|c|c|c|}
			\hline
			\textbf{System}              & \textbf{Method} & \textbf{Accuracy}                & \textbf{Precision}               & \textbf{Recall}                  & \textbf{F1}                      \\ \hline
			\multirow{2}{*}{\textit{S1}} & RF     & $1.000 \pm 0.000 \bigcdot$ & $1.000 \pm 0.000 \bigcdot$ & $1.000 \pm 0.000 \bigcdot$ & $1.000 \pm 0.000 \bigcdot$ \\ \cline{2-6} 
			& SVM    & $0.999 \pm 0.002$       & $0.999 \pm 0.002$       & $0.999 \pm 0.002$       & $0.999 \pm 0.002$       \\ \hline
			\multirow{2}{*}{\textit{S2}} & RF     & $0.999 \pm 0.002 \bigcdot$ & $0.999 \pm 0.002 \bigcdot$ & $0.999 \pm 0.002 \bigcdot$ & $0.999 \pm 0.002 \bigcdot$ \\ \cline{2-6} 
			& SVM    & $0.990 \pm 0.018$       & $0.991 \pm 0.016$       & $0.990 \pm 0.018$       & $0.990\pm 0.018$        \\ \hline
		\end{tabular}
	}
\end{table}
Both the RF and SVM yielded superior performance.

\section{Limitations}
\label{section:discussion}
In this section, we address the potential limitation of our proposed approach.
\subsection{Zero-day cryptocurrencies} 
A zero-day cryptocurrency 
\par
Importantly, miners prefer (as presented in Section~\ref{section:evaluation}) 

\subsection{Scalability}
The key

\section{Conclusion}
\label{section:conclusion}
Cybercriminals have developed
\par
We keep such investigation as part of our future work. We also hope to release a desktop application for run-time identification of covert cryptomining.
%\ankit{In the future, we will investigate the impact of samples from different operating system and virtualized environments.} We also hope to release a desktop application for run-time identification of covert cryptomining

\section*{Acknowledgment}
Ankit Gangwal is pursuing his Ph.D. with a fellowship for international students funded by Fondazione Cassa di Risparmio di Padova e Rovigo~(CARIPARO). This work was supported in part by EU LOCARD Project under Grant H2020-SU-SEC-2018-832735, and in part by Huawei Project ``Secure Remote OTA Updates for In-Vehicle Software Systems'' under Grant HIRPO 2018040400359-2018.%This work is partially supported by the EU TagItSmart! Project (agreement H2020-ICT30-2015-688061), the EU-India REACH Project (agreement ICI+/2014/342-896), the grant n. 2017-166478 (3696) from Cisco University Research Program Fund and Silicon Valley Community Foundation, and by the grant ``Scalable IoT Management and Key security aspects in 5G systems'' from~Intel.

%\balance
\bibliographystyle{IEEEtran}
\bibliography{bib_full}
%\balance

%\appendices
%\section{Proof of the First Zonklar Equation}
%Appendix one text goes here.
%
%title for an appendix
%% if you want by leaving the argument blank
%\section{}
%Appendix two text goes here.

\appendices
\counterwithin{table}{section}
\renewcommand{\thesection}{\Alph{section}}%
% or try \arabic{section}

\section{Acronyms}
%\section{Acronym used for various cryptocurrencies}
\label{appendix_a}

\tablename{~\ref{table:acronym}} describes the acronyms used for different cryptocurrencies.
\begin{table}[H]
	\centering
	\caption{Cryptocurrencies and their acronym}
	\label{table:acronym}
	\begin{tabular}{|c|c|}
		\hline
		\textbf{Acronym} & \textbf{Cryptocurrency} \\ \hline
		BCD              & Bitcoin Diamond        \\ \hline
		BCH              & Bitcoin Cash           \\ \hline
		BTC              & Bitcoin                \\ \hline
		BTM              & Bytom                  \\ \hline
		DASH             & Dash                   \\ \hline
		DCR              & Decred                 \\ \hline
		ETC              & Ethereum Classic       \\ \hline
		ETH              & Ethereum               \\ \hline
		LTC              & Litecoin               \\ \hline
		QRK              & Quark                  \\ \hline
		SBTC             & SuperBitcoin           \\ \hline
		SC               & Siacoin                \\ \hline%%%%%%%%%%%%NOT CONSIDERED%%%%
		UBTC             & UnitedBitcoin          \\ \hline
		XMC              & Monero-Classic         \\ \hline
		XMR              & Monero                 \\ \hline
		XZC              & Zcoin                  \\ \hline
		ZEC              & Zcash                  \\ \hline
	\end{tabular}
\end{table}

\section{Standard definitions}
\label{appendix_b}
Here, we present the definitions of some concepts that we used in our work.
\begin{description}[\IEEEsetlabelwidth{ABCDEFGHI}\IEEEusemathlabelsep]
	%		\item[MinMax scaler] scales each feature in the range [0,1]. Specifically, given a feature $x$ and one of its assumed value $x_i$ the following formula is applied:
	%		$$
	%		\textit{minmax}(x_i) = \frac{x_i - \textit{min}(x)}{\textit{max}(x)-\textit{min}(x)},
	%		$$
	%		where $\textit{min}(x)$ and $\textit{max}(x)$ are the minimum and maximum value of the feature $x$ in the dataset.
	%		
	\item[Standard scaler] transforms each feature in such a way that the mean becomes zero and standard deviation becomes one. Specifically, given a feature $x$ and one of its value $x_i$, the following formula is applied:
	$$
	\textit{Z}(x_i) = \frac{x_i - \mu(x)}{\sigma(x)},
	$$
	%where $\mu(x)$ is the mean value of the variable $x$ and $\sigma(x)$ its standard deviation.
	where $\mu(x)$ and $\sigma(x)$ are the mean and standard deviation of the variable $x$.
	
	\item[Standard error] of a variable $y$ is expressed as:
	$$
	S_E(y) = \frac{\sigma(y)}{\sqrt{n}},
	$$
	where $n$ and $\sigma(y)$ are the number of observations and standard deviation of the variable $y$.
	
	\item[Margin of error] is the range of values above and below the sample mean for a given confidence interval. It is calculated as:
	$$
	z * S_E(y),
	$$
	where $z$ is the coefficient for the selected confidence level. \Eg $z$ is 1.96 for 95\% confidence interval.
	
	\item[Accuracy] measures how often the classifier makes the right prediction defined as the ratio between the number of hit and the number of predictions.
	
	\item[Precision] quantifies the ability of a classifier to not label a negative example as positive. It is computed as the ratio of the number of true positives and the total number of instances labeled as positives.
	
	\item[Recall] defines the probability that a positive prediction made by the classifier is actually positive. It is computed as the ratio of the number of true positives and the total number of positives in the set.
	
	\item[F$_1$~score] is a single metric that combines both precision and recall via their harmonic mean:
	$$
	F_1~score = 2 \times \frac{\textit{precision} \times \textit{recall}}{\textit{precision} + \textit{recall}}
	$$
\end{description}

\iffalse
	\begin{figure}[H]
		\centering
		\includegraphics[trim = 0mm 0mm 0mm 0mm, clip, width=.6\linewidth]{./images/address.pdf}
		\caption[]{Converting a public key into a Bitcoin address}
		\label{figure:address}
	\end{figure}
\fi

\section{Parameters selected by grid search}
\label{appendix_grid_search}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
Here, we list the frequency of paramenter-values 
% biography section

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip
		]{./authors/gangwal}}]{Ankit Gangwal} received his BTech degree in Information Technology from RTU Kota, India in 2011 and his MTech degree in Computer Engineering from MNIT Jaipur, India in 2016. Currently, he is a Ph.D. student in the Department of Mathematics, University of Padua, Italy with a fellowship for international students funded by Fondazione Cassa di Risparmio di Padova e Rovigo (CARIPARO). His current research interest is in the area of security and privacy of the blockchain technology and novel network architectures.%, in particular, Software Defined Networks (SDN).
\end{IEEEbiography}
%\enlargethispage{\baselineskip}
\balance
